Evaluating Complex Queries on Streaming Graphs

We study the problem of evaluating persistent queries over streaming graphs in a principled fashion. These queries need to be evaluated over unbounded and very high speed graph streams. We define a streaming graph data model and query model incorporating navigational queries, subgraph queries and paths as first-class citizens. To support this full-fledged query model we develop a streaming graph algebra that describes the precise semantics of persistent graph queries with their complex constructs. We present transformation rules and describe query formulation and plan generation for persistent graph queries over streaming graphs. Our implementation of a streaming graph query processor shows the feasibility of our approach and allows us to gauge the high performance gains obtained for query processing over streaming graphs.

==> operators.tex <==

\section{Physical Algebra}
\label{sec:physical-algebra}

This section introduces a physical operator algebra for SGA that consists of non-blocking algorithms as physical operator implementations.
%, including a novel algorithm for \textsf{PATH}.
The intuition behind our physical algebra is the following: in the absence of explicit deletions, expirations from windows and result set exhibit a temporal pattern in the way that streaming graph tuples are inserted.
We show that utilizing this pattern enables novel algorithms for query processing and window maintenance.
We also describe how to handle explicit deletions using \textit{negative tuples} for applications that require explicit deletions of previously inserted edges. 

% This section presents a concrete implementation of a physical operator algebra that can be used for persistent evaluation of SGQ (Definition \ref{def:streaming-query}).
% In particular, we first describe how to leverage existing streaming algorithms in literature as physical operator implementations, then introduce a novel algorithm for the path navigation operator.
% %that addresses the limitations of existing approaches.
% The intuition behind our proposed algorithm is that, in the absence of explicit deletions, expirations from windows and outputs exhibit a temporal pattern in the way that streaming graph tuples are inserted.
% We show that utilizing this pattern enables novel algorithms for query processing and window maintenance.

%A naive approach to evaluate persistent queries is \textit{re-evaluation}, where the corresponding one-time query is evaluated over the entire input at every time instant, perhaps with tremendous redundancy.
As noted earlier, our focus is on \textit{incremental} evaluation of persistent queries where the goal is to avoid re-computation of the entire result by only computing the changes to the output as new input arrives.
It is desired that physical operators of a streaming system have non-blocking behaviour, i.e., they do not need the entire input to be available before producing the first result.
Operators with blocking behaviour, such as set difference and nested loop joins, can be unblocked by restricting their range to a finite subset of an unbounded stream \cite{golabo03a, bbd+02}.
Hence, sliding windows that are used to restrict the scope of queries to recent data, a desired feature in many streaming applications, provide a tool for incremental computation of such operators over unbounded streams.
Algorithms we describe here constitute non-blocking, incremental implementations of operators in our streaming graph algebra consistent with the semantics (Section \ref{sec:algebra}). 
Of course, these are not the only physical operator implementations that are possible for SGA; other implementations can possibly be developed, and these are exemplars to demonstrate the implementability of the SGA operators.
They are also what we use in the experiments.

The standard implementations of stateless operators \textsf{FILTER} and \textsf{UNION} can be directly used in SGA.
Similarly, \textsf{WSCAN} is a stateless operator that can be implemented using the standard \textit{map} operator that adjusts the validity interval of an sgt according to the given window specification.

We focus on the stateful operators \textsf{PATTERN} and \textsf{PATH} that need to maintain an internal operator state that is accessed during query processing. This state is updated as new sgts enter the window and old sgts expire.
As discussed earlier, time-based sliding windows ensure that the portion of the input that may contribute to any future result is finite, making incremental, non-blocking computation possible.

\subsection{Pattern matching}
\label{sec:pattern-operator}

Implementation of \textsf{PATTERN} models subgraph patterns as conjunctive queries that can be evaluated using a series of joins. There is a rich literature of streaming join implementations that can be used.
%
%We utilize the rich literature on streaming joins for a non-blocking implementation of \textsf{PATTERN} operator (Definition  \ref{def:subgraph-pattern-operator}) by representing subgraph patterns as conjunctive queries, which can be evaluated using a series of joins.
Symmetric hash join ~\cite{wilschut91}
%Pipelined hash join ~\cite{urhanf2000} 
is commonly used to implement non-blocking joins in the streaming model: a hash table is built for each input stream and upon arrival (expiration) of a tuple, it is inserted into (removed from) its corresponding hash table and other tables are probed for matches \cite{urhanf2000, vldb03_golabo03}.
% This use of explicit deletions to signal expirations corresponds to the \textit{negative tuple} approach.
This produces an append-only stream of results for internal windows that do not invalidate previously reported results upon expiration of their participating tuples \cite{golab:2006yq}.
For external windows that require eviction of old results as the windows slide forward, 
%In the absence of explicit deletions, a join result expires when one of its participating tuples expire.
% Hence, 
expired results can be determined by maintaining expiration timestamps: a join result expires when one of its participating tuples expire.
Our use of validity intervals enables the user or the application to adopt both window semantics without the need for explicit processing of expired input tuples.
%, eliminating the need for explicit processing of expired input tuples.
%, which is equal to the minimum expiration timestamp of its participating tuples, rendering the \textit{direct} approach possible.

Given a subgraph pattern, we take the standard approach of creating a binary join tree where leafs represent streaming graphs as input streams and internal nodes represent pipelined hash join operators.
For instance, Figure \ref{fig:physical-join} shows the join tree for \textsf{PATTERN} of SGQ $Q_1$ whose logical plan is given in Figure \ref{fig:logical-plan}.
We leave the problem of finding efficient join plans (e.g. using  \textit{worst-case optimal joins} \cite{Ngo_2014}) for subgraph pattern queries over streaming graphs as a future work and use the ordering of subgraph pattern predicates given in the query.
%Recently, a new class of join algorithms, \textit{worst-case optimal joins}, is shown to have provably better bounds on cyclic conjunctive queries \cite{Ngo_2014}, and Ammar et al. study subgraph pattern matching over dynamic graphs \cite{vldb18_AmmarMSJ18}.
%Such algorithms can be adapted for cyclic subgraph pattern queries over sliding windows over streaming graphs, but this is out of the scope for this paper.


\begin{figure}
\centering
    \includegraphics[height=2in]{figures/physical-join2.pdf}
    \caption{The join tree that consists of binary hash joins for the \textsf{PATTERN} operator of the logical plan given in Figure \ref{fig:logical-plan}.}
    \label{fig:physical-join}
\end{figure}


% In following, we present non-blocking implementations for the stateful operators of our algebra on sliding windows over streaming graphs, i.e., subgraph pattern matching (Definition \ref{def:subgraph-pattern-operator}) and path navigation (Definition \ref{def:path-navigation-operator}).
% We first describe how to utilize existing literature on streaming joins for subgraph pattern matching on sliding windows over streaming graphs, then introduce our novel non-blocking algorithm for path navigation.


% \subsection{Subgraph Pattern Matching}
% \label{sec:subgraph-pattern}
% We utilize the rich literature on streaming joins for a non-blocking implementation of the subgraph pattern operator of our algebra (Definition  \ref{def:subgraph-pattern-operator}) by representing subgraph patterns as conjunctive queries, which can be evaluated using a series of joins.
% Pipelined hash join ~\cite{urhanf2000} is commonly used in literature to implement streaming joins: a hash table is built for each input stream and upon arrival (expiration) of a tuple, it is inserted into (removed form) its corresponding hash table and other tables are probed for matches.
% This use of explicit deletions to signal expirations corresponds to the \textit{negative tuple} approach.
% In the absence of explicit deletions, a resulting tuple expires when one of its participating tuples.
% Hence, expired results can be determined by their expiration timestamp, which is equal to the minimum expiration timestamp of its participating tuples, rendering the \textit{direct} approach possible.
% Given a subgraph pattern, we take the standard approach of creating a binary join tree where leafs represent streaming graphs as input streams and internal nodes represent pipelined hash join operators.
% We leave the problem of finding efficient join orders for subgraph pattern queries over streaming graphs as a future work and use the ordering of input streaming graphs in the query.

% Recently, a new class of join algorithms, \textit{worst-case optimal joins}, is shown to have provably better bounds on cyclic conjunctive queries \cite{Ngo_2014}.
% Such algorithms can be adapted for cyclic subgraph pattern queries over streaming graphs, but this is out of the scope for this paper.

\subsection{Path Navigation}
\label{sec:path-navigation-implementation}
%We now present a novel algorithm \textit{Streaming Path Navigation} (SPN) that can be used as a physical operator for the \textsf{PATH} operator (Definition \ref{def:path-navigation-operator}). 
% based on the \textit{direct} approach.
The semantics of \textsf{PATH} follows the RPQ model, which specifies path constraints as a regular expression over the alphabet of edge labels and checks whether a path exists with a label that satisfies the given regular expression  \cite{mendelzon1995finding, baeza13}. We propose the \textit{Streaming Path Navigation} \textbf{\ref{alg:arbitrary}} algorithm as a physical operator implementation of \textsf{PATH}.
\textbf{\ref{alg:arbitrary}} follows the automata-based RPQ evaluation strategy \cite{mendelzon1995finding, Pacaci_2020} using the arbitrary path semantics as discussed in Section \ref{sec:algebra}.

\input{algorithms/arbitrary-window}

Algorithm \textbf{\ref{alg:arbitrary}} incrementally performs a traversal of the underlying snapshot graph under the constraints of a given RPQ as sgts arrive.
It first constructs a DFA from the regular expression of a \textsf{PATH} operator, and initializes a spanning forest-based data structure, called $\Delta^W$, that is used as the internal operator state during query processing.
$\Delta^W$ is used to maintain a path segment, i.e., a partial result, between each pair of vertices in the form a spanning forest under the constraints of a given RPQ, consistent with Definition \ref{def:path-navigation-operator}.
Upon the arrival of an sgt, Algorithm \textbf{\ref{alg:arbitrary}} probes $\Delta^W$ to retrieve partial path segments that can be extended with the edge (or a path segment) of the incoming sgt.
Each partial path segment is extended with the incoming sgt, and Algorithm \textbf{\ref{alg:arbitrary}} traverses the snapshot graph $G_{t}$ until no further expansion is possible.

\begin{definition}[Spanning Tree $T_x$]\label{def:spanning-tree}
Given an automaton $A$ for the regular expression $R$ of a \textsf{PATH} operator $\mathcal{P}^R_d$ and a streaming graph $S$ at time $t$, a spanning tree $T_x$ forms a compact representation of valid path segments that are reachable from the vertex $x \in G_{t}$ under the constraints of a given RPQ, i.e., a vertex-state pair $(u,s)$ is in $T_x$ at time $t$ if there exists a path $p \in G_{t}$ from $x$ to $u$ with label $\phi^p(p)$ such that $s = \delta^*(s_0, \phi^p(p))$.
\end{definition}

A node $(u,s) \in T_x$ indicates that there is a path $p$ in the snapshot graph with label $\phi^p(p)$ such that $s = \delta^*(s_0, \phi^p(p))$, and this path can simply be constructed by following parent pointers ($(u,s).pt$) in $T_x$.
Under the arbitrary path semantics, there are potentially infinitely many path segments between a pair of vertices that conform to a given RPQ due to the presence of cycles in the snapshot graph and a Kleene star in the given RPQ.
Among those, \ref{alg:arbitrary} materializes the path segment with the largest expiry timestamp, that is, the path segment that will expire furthest in the future. 
Consequently, for each node $(u,s) \in T_x$, the sequence of vertices in the path from the root node to $(u,s)$ corresponds to the path from $x$ to $u$ in the snapshot graph with the largest expiry timestamp. 
This is achieved by the coalesce primitive (Definition \ref{def:coalesce}) with an aggregation function \texttt{max} over the expiry timestamp of path segments. \footnote{Arbitrary path semantics provides the flexibility for the aggregation function $f_{agg}$ of the coalesce primitive.}
Upon expiration of a node $(u,s)$ in $T_x$ and its corresponding path segment in the snapshot graph, this guarantees that there cannot be an alternative path segment between $x$ and $u$ that have not yet expired.
Hence, we can \textit{directly} find expired tuples based on their expiry timestamps.
% Hence, the expiry timestamp $(u,s).exp$ of $(u,s) \in T_x$ is equal to the largest expiry timestamp of all paths between vertices $x$ and $u$ with label $\phi^p(p)$ such that $s = \delta^*(s_0, \phi^p(p))$.
This is based on the observation that expirations have a temporal order unlike explicit deletions, and \ref{alg:arbitrary} utilizes these temporal patterns to simplify window maintenance.

\begin{definition}[$\Delta^W$ Index]\label{def:delta}
Given an automaton $A$ for the regular expression $R$ of a \textsf{PATH} operator $\mathcal{P}^R_d$ and a streaming graph $S$ at time $t$, $\Delta^W$ is a collection of spanning trees (Definition \ref{def:spanning-tree}) where each tree $T_x$ is rooted at a vertex  $x \in G_{t}$ for which there is an sgt $t \in S(t)$ with a label $l$ such that $\delta(s_0, l) \neq \emptyset$ and $src=x$.
\end{definition}

$\Delta^W$ encodes a single entry for each pair of vertices under the constraints of a given query, consistent with the set semantics of snapshot graphs (Section \ref{sec:data-model}). 
Due to spanning-tree construction (Definition \ref{def:spanning-tree}), actual paths can easily be recovered by following the parent pointers; hence, $\Delta^W$ constitutes a compact representation of intermediate results for path navigation queries over materialized path graphs.
Our implementation models $\Delta^W$ as a hash-based inverted index from vertex-state pairs to spanning trees, enabling quick look-up to locate all spanning trees that contain a particular vertex-state pair.
Upon arrival of an sgt $t=(u,v,l, [ts, exp), \mathcal{D})$, Algorithm \textbf{\ref{alg:arbitrary}} probes this inverted index of $\Delta^W$ to retrieve all path segments that can be extended with the incoming sgt, that is, spanning trees that have the node $(u,s)$ with an expiry timestamp smaller than $ts$ for any state $s \in \{ s \in S \mid \delta(s,l) \neq \emptyset \}$ (Line \ref{line:expandable_trees}).
If the target node $(v,t)$ for $t=\delta(s,l)$ is not in the spanning tree $T_x$, Algorithm \textbf{\ref{alg:insertrapq_insert_edge}} is invoked to expand the existing path segment from $(x,0)$ to $(u,s)$ with the node $(v,t)$ and to create a new leaf node as a child of $(u,s)$.
In case there already exists a path segment between vertices $(x,0)$ and $(v,t)$ in $\Delta^W$, i.e., the target node $(v,t)$ is already in $T_x$, Algorithm \textbf{\ref{alg:arbitrary}} compares its expiry timestamp with the new candidate (Line \ref{line:insertrapq_updateexpiry}).
If the extension of the existing path segment from $(x,0)$ to $(u,s)$ with $(v,t)$ results in a larger expiry timestamp than $(v,t).exp$, Algorithm \textbf{\ref{alg:updaterapq_update_subtree}} is invoked to update the expiry timestamp of $(v,t)$ and its children in $T_x$.
Algorithms \textbf{\ref{alg:insertrapq_insert_edge}} and \textbf{\ref{alg:updaterapq_update_subtree}} traverse the snapshot graph until no further update is possible.
The following example illustrates the behaviour of Algorithm \textbf{\ref{alg:arbitrary}} on our running example.

\begin{example}\label{ex:navigation_algorithm}
Consider the real-time notification query in Example \ref{ex:alert} whose SGA expression is given in Example \ref{ex:canonical_form}.
Figure \ref{fig:stream-horizontal} shows an excerpt of the streaming graph input to the \textsf{PATH} operator $\mathcal{P}^{RL^+}_{RLP}$.
Figure \ref{fig:tree-v1} depicts a spanning tree $T_x \in \Delta^W$ at $t = 27$.
Upon arrival of the sgt $(y,u,RL,[28,37), \mathcal{D} = \{(y,RL,u)\})$ at $t=28$, Algorithm \textbf{\ref{alg:arbitrary}} extends the path segment from $(x,0)$ to $(y,1)$ with $(u,1)$, and compares its expiry timestamp with that of $(u,1)$ that is already in $T_x$. 
As the new extension has larger expiry timestamp, the validity interval and the parent pointer of $(u,1) \in T_x$ is updated (Line \ref{line:insertrapq_updateexpiry} in Algorithm \textbf{\ref{alg:arbitrary}}).
Then, incoming sgts at times $t=28$ and $t=29$ are processed by Algorithm \textbf{\ref{alg:insertrapq_insert_edge}} as corresponding target nodes $(v,1)$ and $(s,1)$ are not in $T_x$, adding $(v,1)$ and $(s,1)$ as children of $(u,1)$.
At $t=30$, the incoming sgt $(w,v,RL,[30,39), \mathcal{D} = \{(w,RL,v)\})$ might extend the path segment from $(x,0)$ to $(v,1)$ with expiry timestamp 33.
However, Algorithm \textbf{\ref{alg:arbitrary}} does not make any modification to $\Delta^W$, as $(v,1)$ is already in $T_x$ with a larger timestamp (Line \ref{line:insertrapq_updateexpiry}).
Figure \ref{fig:tree-v2-new} depicts the resulting spanning tree $T_x$ at $t=30$.
\end{example}


\begin{figure*}
    \centering
    \begin{subfigure}[t]{0.35\textwidth}
        \includegraphics[width=\textwidth]{figures/stream-horizontal2.pdf}
        \caption{Streaming Graph $S$}
        \label{fig:stream-horizontal}
    \end{subfigure}
    \begin{subfigure}[t]{0.17\textwidth}
        \includegraphics[width=\textwidth]{figures/tree-v1.pdf}
        \caption{$t$ = 27}
        \label{fig:tree-v1}
    \end{subfigure}
        \begin{subfigure}[t]{0.18\textwidth}
        \includegraphics[width=\textwidth]{figures/tree-v2-new.pdf}
        \caption{$t$ = 30}
        \label{fig:tree-v2-new}
    \end{subfigure}
    \begin{subfigure}[t]{0.18\textwidth}
        \includegraphics[width=\textwidth]{figures/tree-v2-old.pdf}
        \caption{$t$ = 30 for \cite{Pacaci_2020}}
        \label{fig:tree-v2-old}
    \end{subfigure}
    \caption{(a) A streaming graph $S_{RLP}$ as the input for \textsf{PATH} operator, (b) spanning tree $T_x$ at $t = 28$, (c) spanning tree $T_x$ at $t = 30$ of the proposed algorithm following the \textit{direct} approach, and (d) spanning tree $T_x$ at $t = 30$ of \cite{Pacaci_2020} following the \textit{negative tuple} approach.}
    \label{fig:expiry-example}
    %\vspace{-0.8cm}
\end{figure*}


As described earlier, $\Delta^W$ stores a \textit{parent} pointer for each node pointing to its parent node in the corresponding spanning tree, and  
Algorithm \textbf{\ref{alg:updaterapq_update_subtree}} updates these pointers during processing.
By traversing these parent pointers for each resulting sgt, Algorithm \textbf{\ref{alg:insertrapq_insert_edge}} can construct the actual path (Line \ref{line:addresult}) and return it as a part of the resulting sgt, i.e., it populates the implicit payload attribute $\mathcal{D}$ of the resulting sgt with the sequence of edges that forms the resulting path.
The cost of this operation is $\mathcal{O}(l)$ where $l$ is the length of the resulting path.

$\Delta^W$ guarantees that the expiry timestamp of a node $(u,s)$ in $T_x$ is equal to largest expiry timestamp of all paths between $x$ and $u$ in the snapshot graph with a label $l$ such that $s = \delta^*(s_0, l)$.
Consequently, for a node $(u,s) \in T_x$  with expiry timestamp smaller than $t$, there cannot be another path from $x$ to $u$ with an equivalent label that is valid at time $t$.
Consider the spanning tree given in Figure \ref{fig:tree-v2-new}.
Algorithm \textbf{\ref{alg:arbitrary}} can directly determine, without additional processing, that nodes $(z,1)$ and $(t,1)$ are expired as their expiry timestamp is 31.
Thus, at any given time $t$, Algorithm \textbf{\ref{alg:arbitrary}} can simply ignore a node $(u,s) \in T_x$  with expiry timestamps smaller than $t$ (Line \ref{line:insertrapq_updateexpiry}) and such nodes can be removed from $\Delta^W$.
To prevent $\Delta^W$ from growing unboundedly due to expired tuples, a background process periodically purges expired tuples from $\Delta^W$.


% \todo{This can be efficiently computed using a Dijkstra-style traversal with}
% detailed description of direct vs nt on a running example
%\input{direct-vs-nt}

\subsection{Explicit Deletions}
\label{sec:explicit-deletions}

Physical implementations of \textsf{PATTERN} and \textsf{PATH} rely on the \textit{direct} approach that utilizes the temporal pattern of sliding windows for state maintenance; the expiration timestamps are used to \textit{directly} locate expired tuples.
On append-only streaming graphs, existing sgts only expire due to window movements.
Albeit rare, certain applications might require explicit deletions of previously inserted sgts, which necessitates the use of the \textit{negative tuple} approach to handle such explicit deletions.\footnote{The \textit{negative tuple} approach  can also be used to signal expirations through an explicit deletion of the corresponding sgt to undo its effect \cite{ghanem2006incremental, golabo05, Pacaci_2020}. 
Indeed, the negative-tuple approach can be used for incremental evaluation of an arbitrary computation, whereas direct approach is applicable to negation-free queries over append-only streaming graphs \cite{golabo05}.}
Deleted sgt, with an additional flag to denote deletion -- i.e., a negative tuple, is used to undo the effect of the original sgt on the operator state and to invalidate previously reported results, if necessary.
For pipelined hash join, which is used in the implementation of \textsf{PATTERN}, processing of negative tuples is the same as original input tuples: a negative tuple is removed from its corresponding hash table and other tables are probed to find corresponding deleted results.


% Path navigation operator requires additional processing for explicit deletions due to presence of multiple paths between a pair of vertices.

Similarly, we adopt the \textit{negative tuple} approach for explicit deletions of sgts in \textsf{PATH} operator.
%, which was first introduced in \cite{Pacaci_2020}.
In brief, upon explicit deletion of an sgt, we first identify tree-edges that disconnect spanning trees in $\Delta^W$. 
For each such tree-edge, we first mark the nodes in the subtree that are disconnected due to the explicit deletion.
Then, for each node in this subtree, we use a Dijkstra-based traversal over the snapshot graph to find an alternative path with the largest expiry timestamp.
Dijkstra's algorithm guarantees that we can efficiently find the path with the largest expiry timestamp for each marked node, consistent with Definition \ref{def:delta}.
A marked node is removed from the spanning tree only if there is no alternative valid path.
Deletion of a non-tree edge does not require any modification as it leaves spanning trees unchanged.
The use of negative tuples for explicit deletions in the context of RPQ evaluation is first proposed by Pacaci et al \cite{Pacaci_2020}.
However, that technique uses the \textit{negative tuple} approach for both explicit deletions and window management, i.e., processing of expired sgts due to sliding window movements. 
This is in contrast to our strategy of utilizing the validity intervals of path segments in $\Delta^W$ index to \textit{directly} locate expired tuples, which simplifies the window management by eliminating the need for explicit processing of expired sgts.



